Hey Robot! Personalizing Robot Navigation through Model Predictive Control with a Large Language Model

Robot navigation methods allow mobile robots to operate in applications such as warehouses or hospitals. While the environment in which the robot operates imposes requirements on its navigation behavior, most existing methods do not allow the end-user to configure the robot's behavior and priorities, possibly leading to undesirable behavior (e.g., fast driving in a hospital). We propose a novel approach to adapt robot motion behavior based on natural language instructions provided by the end-user. Our zero-shot method uses an existing Visual Language Model to interpret a user text query or an image of the environment. This information is used to generate the cost function and reconfigure the parameters of a Model Predictive Controller, translating the user's instruction to the robot's motion behavior. This allows our method to safely and effectively navigate in dynamic and challenging environments. We extensively evaluate our method's individual components and demonstrate the effectiveness of our method on a ground robot in simulation and real-world experiments, and across a variety of environments and user specifications.

==> draft/experiments_design.tex <==
\section{Experiments design (Initial idea)}

For A, we may create a python file that prompts the respective assistant and we could manually evaluate the outputs under several repetitions.\\
For B and possibly C, I am setting up dvc that defines a set of experiments that are run continuously after each other. I would test over a set of prompts and environments and collect the resulting navigation metrics in a table. For now, I would consider a corridor and open space environment, maybe I will add one more environment that is a bit more involved.

\subsection{Assistants capabilities}
This experiment would be about defining queries and getting the number of times the queries are fulfilled. We should define the list of queries to be included. We could have different subexperiments:
\subsubsection{Capability assistant:} If the cost can do one thing, check if it may understand its capabilities:
\begin{itemize}
    \item Having a cost that follows a reference path: \textit{Go to the goal}, \textit{Follow the path}, \textit{Follow the closest human}, \textit{Go to the goal while keeping more than 1 m from humans}, \textit{Stick to the path}.
    \item Having a cost that goes to the goal: \textit{Go to the goal}, \textit{Follow the path}, \textit{Follow the closest human}, \textit{Go to the goal while keeping more than 1 m from humans}, \textit{Stick to the path}.
    \item Having a cost that follows a human: \textit{Go to the goal}, \textit{Follow the path}, \textit{Follow the closest human}, \textit{Go to the goal while keeping more than 1 m from humans}, \textit{Stick to the path}.
\end{itemize}

\subsubsection{Cost generation assistant:} Check if the generated code is what specified by the input:
\begin{itemize}
    \item \textit{Follow the path.}
    \item \textit{Reach the goal}.
    \item \textit{Follow the closest human.}
    \item \textit{Reach the goal while trying to keep a safe distance from humans.}
    \item \textit{Reach the goal as fast as possible.}
\end{itemize}

\subsubsection{Weight assistant:} Having a cost that can fulfill the task, check whether the parameters set make sense with the behavior queried by the user:
\begin{itemize}
    \item \textit{Be faster.}
    \item \textit{Be slower.}
    \item \textit{Stick to the path.}
    \item \textit{Be smoother.}
    \item \textit{Take more distance to humans.}
\end{itemize}

\subsection{Qualitative scenario plots}

In this experiment, we may have the same dynamic scenario for different queries, having a plot of what the robot did for each query specification, having clearly different specifications. The queries may be:
\begin{itemize}
    \item Follow the path.
    \item Stick to the path as much as possible.
    \item Follow the path while trying to be at least 1 m far from humans.
    \item Follow the closest human.
    \item You are driving in a hospital
    \item You are driving in a factory. There are no humans around.
\end{itemize}

\subsection{Qualitative scenario video}

In two or three different environments, have a list of queries that are formulated each 5-10 seconds one after other (also check the generation time). Record a video of the system properly accounting for each query while we show the query working in real time.

\subsection{Qualitative ground-robot experiment}

Have some external people randomly telling the robot what to do. It can be done with the Jackal (Delft) or in Zaragoza (probably with a Turtlebot 2).

\subsection{Real world exps}

2 or 3 people
Goals that are generated in the two corners of the room.
Calibrate the camera with points and the helmet.
Change velocity of the robot and constraints.

\begin{itemize}
    \item Reach the goal.
    \item Adapt to the environment (save photo).
    \item Be slower.
    \item Be as fast as you can.
    \item Increase acceleration and rotation capabilities.
    \item Be smoother.
    \item Reach the goal while keeping a safe distance of the humans.
    \item The safe distance must be of two meters.
    \item Follow the closest human while keeping a safe distance to him.
    \item Reach the goal as fast as possible.
    \item Try to be as smooth as you can.
\end{itemize}

==> draft/idea.tex <==
\section{Introduction (Initial idea)}

\subsection{Motivation}
Trajectory optimization methods are effective for mobile navigation among humans. However, socially aware navigation is tied to the situation and user intentions and this context must be provided to the planner (e.g., modifying the tuning and shape of the cost function) to achieve satisfactory performance.
% Thus, a social behavior relies largely on specific tuning and shape of the cost function. 

Existing work in social navigation has limited success in controlled environments, but typically fails to generalize. For example they may learn inputs directly from simulation (Reinforcement Learning) or learn high-level inputs from human walking data (e.g., homology classes of interaction or a cost-to-go). Methods that tune the MPC using bayesian optimization, are also limited to the environment where the weights are optimized.

% More detailed version
%Work in offline Reinforcement Learning, for example, tries to learn the robot inputs directly from simulation or real-world data where the robot interacts with pedestrians, but its behavior is fully tied to the specific environment. In addition, safely behavior in an unexplored part of the state space that the data did not cover is not guaranteed. Another approach is to learn high-level inputs (e.g., homology classes of interaction or a cost-to-go) or tune the cost function of the MPC using e.g., bayesian optimization. While these methods, relying on trajectory optimization, are safer by construction, their decision-making do not generalize to \textit{any} setting and are still dependent on the situation used for the tuning; while having enough data to make it roboust for every possible situation is intractable.

Instead of learning the planner behavior in general, in this paper, our goal is to develop an MPC planner that can adapt to any situation using sensor and user input as cues, by using the social understanding of Large Language Models (LLMs). In this way, the user does not need expert knowledge about robotics to tell the robot how to behave. We consider both behavior specification and task assignment.

\textit{Behavior specification: } Our approach allows the robot for example, to slow down in a hospital or restaurant, while speeding-up in a controlled warehouse setting, or allows it to move smoother if the user thinks its motion is too jerky. 

\textit{Task Assignment} The robot may have to drive to a goal, follow a path or follow an object and we allow the user to specify this to the robot. Our aim is to let the user specify these directions, allowing the robot to generalize to any setting through additional instructions provided online.

\subsection{Contribution}
We present an autonomous planning stack that dynamically adapts to user and sensor inputs, enabling the local planner to modify its behavior based on the environment. By integrating knowledge from LLMs, it can leverage the underlying human intuition to operate effectively across a diverse range of scenarios.
To this end, our contributions are:
%We have the following contributions:

\begin{enumerate}
    \item We combine LLM's with a well-established local planner, specifically Model Predictive Control (MPC) to dynamically adapt the cost function maintaining the guarantees provided by the MPC.
%     Our planner adapts to user and sensor inputs to adapt to
% its environment on the fly. This allows our autonomous
% planning stack to adapt its behavior to environments
% that the LLM is aware of and to leverage the underlying
% intuition of humans in a wide range of environments.
    \item To allow for general task assignment, we automatically generate a new cost function when the user's task cannot be achieved by the current optimization solver. The weights of this cost function are tuned by a secondary LLM-based module.
    % \item In addition, by leveraging topology-driven MPC, our method finds multiple local optima and ensures that changes in the tuning of the cost function affect the final solution.    
\end{enumerate}
Our software is written in Python, C++ and ROS and will be released upon acceptance.

\section{Method (Initial idea)}
\textbf{See Fig.~\ref{fig:llm_nav}} for an overview of our assistants (each assistant uses the ChatGPT 4.0 API)

\subsection{What we have}
We have the components as illustrated in Fig.~\ref{fig:llm_nav}. All assistants are working fairly reliably. Some notes:
\begin{enumerate}
    \item By reducing the ChatGPT responses, we can get responses from the API in about $1$s.
    \item To pass the weights to the MPC, we are normalizing all the weights and scaling them by an importance between $0-10$ provided by ChatGPT.
\end{enumerate}

%The \textbf{CapabilityAssistant}, \textbf{EnablingAssistant} and \textbf{WeightAssistant} are working reliably, the other two are work-in-progress. We currently connect the importance of the \textbf{WeightAssistant} to the planner by normalizing the weights and scaling them linearly with their importance. By reducing ChatGPT responses (e.g., not asking for any motivation), we can complete queries in $1$ to $2$ seconds. 

\textit{Main Challenge:} The generation of the cost using ChatGPT needs to know the exact context in which the solver code is written and an understanding of what it can use in an optimization context. This works reasonably well even for complex objectives (e.g., keep at least 1.5m distance from pedestrians and go to the goal) but if it fails to generate the correct objective we currently have no way to verify that. We may try to compile a list of prompts for generating new costs and to report their success rate.

%We currently have a working version offline (first generate the code and then launch everything) but the integration should be straightforward. We also have a way to integrate it with the Enabler and Weight Assistant, so that the generated wrights may be changed (offline too). The limitations of this module are:
% \begin{itemize}
%     \item It needs to interact with GPT, then generate the solver and then compile, so it takes some time (around 1 minute), specially the compilation of the new code.
%     \item Having the inputs we have, maybe defining all cost terms we can think about and then enabling/disabling them weights would produce the same result in less time while guaranteeing robustness.
%     \item We can't guarantee that the cost is going to work as expected. Some prompts always work but some complex ones not always. We can also conduct experiments and tell the success rate of having a correct result out of 10 times of the same prompt, for example.
% \end{itemize}

%We want to check if it makes sense to generate costs using ChatGPT or if enabling/disabling weights is enough. Additionally, we want to check if we can allow ChatGPT to modify the C++ code to change some of the data. For example, so that when the user prompts to follow the nearest pedestrian, ChatGPT can load the nearest pedestrian from the obstacle data as goal of the planner.

\section{Results (Initial idea)}
We would like to test the approach in simulation (environment TBD), verifying that the user can prompt different behaviors from the robot and can modify its task assignment on the fly. E.g., reporting navigation metrics under different user instructions. We would like to find out if there are any prompts that fail and investigate why.

We would like to do real-world experiments with the Jackal and to let participants change the robot behavior using voice commands.

% To do:
% - Find a way to decide if a new cost should be generated from user's prompt or tuning the variables is enough.
% - Refining prompts.
% - The first module currently works in the simulator, but the second does not (it should be straightforward).
% - Simulation experiments that clearly show the changes in behavior.
% - Limitation experiments of getting prompts that fail or usually fail.
% - Maybe real-world experiments.

% - Having a cost that is working, a way to modify it using prompts. We provide information of the weight that are present and what they mean and ask GPT to rate their importance (1 to 10). Then, we normalize it and get the new weighted cost.
% - We can also generate a new cost. We explain to GPT the variables and functions it may use and provide a small example of how to do it. It then generates a new function that is compiled into the code.
% - We also ask GPT of give a description of the weights and use the description to connect to the previous module, so we can simply tune the weights instead of generating new code.




==> draft/todo.tex <==
\section{To-do list}
\begin{itemize}
    \item Make a function to clear the conversation of assistants and use it with only some of them.\Diego{Done.}
    \item Make a list of things to improve, bugs, or things that don't work \Diego{Doing...}
    \item Try to include the camera (wouldn't spend too much time if it's hard) \Diego{Done}
    \item Accurately design the experiments (\Oscar{Oscar: working on this. I am setting up \texttt{dvc} with \texttt{jackal\_socialsim}, so that we can run a few standardized experiments.})
    \item Do the experiments
    \item Write
\end{itemize}

\subsection{Bugs and undesired behavior}
\begin{itemize}
    \item Sometimes the reference velocity is taken as a weight rather than a parameter. Should it be a weight or a parameter? We can specifically include this in the code. We can also manually include the reference velocity in the things it may tune (in get\_weights), so that we can tell it to be slower or faster. Otherwise, it sometimes does it and sometimes doesn't. \Diego{SOLVED}
    \item It is not clear for it what is smoother or not (increasing or decreasing the acceleration and rotational weights) at it is just doing get\_cost and a product. This is a problem if, for example, it is penalizing rotational velocity too much and can't reach the goal because of that. \Oscar{I agree, I think we need to provide some context with regards to social motion planning and what the terms refer to. What do you think?} \Diego{SOLVED}
    \item When we go from go to a goal to follow the path, it sometimes just stops. \Diego{SOLVED}
    \item Todo: Test the cost generation assistant by compiling its generated code. \Diego{SOLVED}
    \item Sometimes there is a behavior that can't be fulfilled with the current cost, and the current behavior/task divider can't answer that. \Diego{SOLVED}
    \item The contouring costs are usually directly preferred over other objectives causing the robot to move slowly and stick to the path completely. \Diego{Is this a problem? I mean you can always say hey, don't stick that much to the path}
    \item Camera is triggered too many times, sometimes weirdly. For example, imagine the robot is randomly pointing towards a wall when the photo is taken. The environment will randomly be "you are in an open space" or "you are in a confined space". Then, it points again to the crowd and changes triggers a new query, messing up user queries. \Diego{SOLVED}
    \item The cost generation prioritizes too much using the shorcut costs. \Diego{SOLVED}
    \item Sometimes there are doubles included as weights in the generated code. \Diego{SOLVED}
    \item Sometimes there are doubles included as weights in the weight retrieval assistant. \Diego{SOLVED}
    \item Remove the navigation settings (self.settings) from the code if they are not longer used. \Diego{SOLVED}
    \item Goal is sometimes added in get\_weights when there is no cost about it.
    \item Currently, the behavior/task assistant is only used to check if it's a query environment. Maybe can be done with the cost capability assistant?
    \item Improve results for the capability assistant.
\end{itemize}
